PrivAudit: A Dual-Lens Auditing Framework for Website Privacy Practices under the CCPA

Five years after the enforcement of the California Consumer Privacy Act (CCPA), understanding how website privacy practices evolve at scale in response to regulation remains a key challenge for both researchers and regulators. Prior work and regulatory efforts have focused on manual and case-specific enforcement, but there remain no scalable approaches to systematically audit two key user-facing facets of websites that are crucial signals for the CCPA: privacy disclosures and front-end user tracking behavior. In this paper, we present PrivAudit, an automated auditing framework that adopts a dual-lens approach to capture: (1) privacy disclosures through large language model-based analysis of privacy policies grounded in CCPA provisions, and (2) user-observable data collection behavior through automated browser measurements of cookie writes under diverse privacy configurations. We apply PrivAudit to 998 websites and report two broad findings. The law is associated with stronger privacy disclosures: CCPA-subject policies are more likely to disclose opt-out mechanisms, data-sharing practices, and user rights. On the other hand, cookie-based tracking remains pervasive, with both CCPA-subject and not-subject websites setting a total of 6,392 targeting cookies, 49% of which are third-party writes. Moreover, cookies show limited-to-moderate responsiveness to privacy signals and consent choices, even when websites claim to honor them in their disclosures. Our results highlight the need for multi-layered and scalable auditing approaches that combine policy analysis with behavioral evidence. PrivAudit can support these auditing workflows at scale by generating actionable signals and patterns for further manual review. We open-source PrivAudit and are engaging with regulators to support auditing in practice.

==> figures/TikZ_figure_for_CCPA_Compliance_Conveyor_Pipeline.tex <==
\usepackage{tikz}
\usetikzlibrary{
  shapes.geometric,
  arrows.meta,
  positioning,
  shadows
}

\tikzset{
  process/.style={
    rectangle,
    rounded corners,
    draw=blue!80,
    fill=blue!10,
    thick,
    text width=4cm,
    align=center,
    minimum height=1.2cm,
    drop shadow
  },
  data/.style={
    trapezium,
    trapezium left angle=70,
    trapezium right angle=110,
    draw=green!70,
    fill=green!10,
    thick,
    text width=3cm,
    align=center,
    minimum height=1cm,
    drop shadow
  },
  fusion/.style={
    diamond,
    draw=red!80,
    fill=red!10,
    thick,
    text width=3.5cm,
    align=center,
    minimum height=1.2cm,
    drop shadow
  },
  arrow/.style={
    -{Latex[length=3mm,width=2mm]},
    thick
  }
}
% ─────────────────────────────────────────────────────────────────────────────

% ─────────────────────────────────────────────────────────────────────────────
% In the body where you want the figure:
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    node distance=8mm and 12mm,
    every node/.style={font=\small}
  ]
    % Left stream: Technical Audit
    \node[process] (selection) {
      Website Selection \& \\ Categorization
    };
    \node[process, below=of selection] (browsing) {
      Automated Browsing \& Cookie Extraction\\(6 Privacy Configs)
    };
    \node[process, below=of browsing] (cookie) {
      Cookie Metadata \\ Classification
    };
    \node[data, below=of cookie] (pvs) {
      Compute \\ Privacy Violation Score
    };

    % Right stream: Policy Audit
    \node[process, right=of selection] (policy) {
      Privacy Policy \\ Extraction
    };
    \node[process, below=of policy] (segmentation) {
      Policy Segmentation \\ \& Embedding
    };
    \node[process, below=of segmentation] (scoring) {
      LLM Rubric-Based \\ Scoring
    };
    \node[data, below=of scoring] (policyscore) {
      Compute \\ Policy Score
    };

    % Fusion and Verdict
    \node[fusion, below=15mm of $(pvs)!0.5!(policyscore)$] (fusion) {
      Fusion Layer \\ (PVS + Policy Score)
    };
    \node[process, below=of fusion] (quadrant) {
      Compliance \\ Quadrants
    };

    % Arrows: Technical stream
    \draw[arrow] (selection) -- (browsing);
    \draw[arrow] (browsing) -- (cookie);
    \draw[arrow] (cookie) -- (pvs);

    % Arrows: Policy stream
    \draw[arrow] (policy) -- (segmentation);
    \draw[arrow] (segmentation) -- (scoring);
    \draw[arrow] (scoring) -- (policyscore);

    % Arrows: Fusion
    \draw[arrow] (pvs) -- (fusion);
    \draw[arrow] (policyscore) -- (fusion);
    \draw[arrow] (fusion) -- (quadrant);
  \end{tikzpicture}
  \caption{Overview of our methodology: two parallel audit streams (technical vs.\ policy) converge in a fusion layer to assign each site to one of four compliance quadrants.}
  \label{fig:methodology-diagram}
\end{figure}
% ─────────────────────────────────────────────────────────────────────────────


==> figures/boxplot-cookie-type-default-ccpa.tex <==
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.85\linewidth]{figures/new_figures/boxplot_default_cookie_types_ccpa_split.pdf}
%     \caption{Distribution of cookie counts per website (Default browsing configuration), split by cookie category. Both \subject and \notsubject websites set a significant number of Targeting cookies.}
%     \label{fig:boxplot-cookie-type-default-ccpa}
% \end{figure}


\begin{figure}[!t]
    \centering
    \includegraphics[width=0.85\linewidth]{figures/new_figures/boxplot_all_configs_cookie_types_ccpa_split.pdf}
    \caption{Distribution of cookie counts per website (Default browsing configuration), split by cookie category. Both \subject and \notsubject websites set a significant number of Targeting cookies.}
    \label{fig:boxplot-cookie-type-default-ccpa}
\end{figure}




==> figures/fig_dual_audit_architecture.tex <==
% ─── Dual-Audit Architecture Figure ─────────────────────────────────────────
\usepackage{tikz}
\usetikzlibrary{
  shapes.geometric,
  arrows.meta,
  positioning,
  shadows
}


\begin{figure}[ht]
\centering
\begin{tikzpicture}[
  node distance = 1.4cm and 2.4cm,
  every node/.style = {align=center, font=\small},
  box/.style     = {rectangle, draw=black, rounded corners,
                    minimum width=3.8cm, minimum height=1.15cm, fill=blue!5},
  fusion/.style  = {rectangle, draw=black, rounded corners,
                    minimum width=4.5cm, minimum height=1.4cm, fill=orange!20},
  flow/.style    = {thick, -{Latex[length=2.3mm,width=1.8mm]}}
]

% ── Input node ────────────────────────────────────────────────────────────────
\node[box] (websites) {Target Websites\\(n = 1\,016)};

% ── Parallel streams ──────────────────────────────────────────────────────────
\node[box, below left=of websites]  (behavioral)
      {Behavioural Stream\\\footnotesize Cookie Extraction \& PVS};
\node[box, below right=of websites] (semantic)
      {Semantic Stream\\\footnotesize LLM Policy Scoring};

% Stream details
\node[below=9mm of behavioral] (bdetails)
      {\footnotesize Puppeteer + GPC/DNT/uBlock\\[-1pt]
       \footnotesize Privacy-Violation Score};
\node[below=9mm of semantic]   (sdetails)
      {\footnotesize GPT-4o \& Gemini-2.5\\[-1pt]
       \footnotesize Completeness, Usability, Accuracy};

% ── Fusion layer ──────────────────────────────────────────────────────────────
\node[fusion, below=3cm of websites] (fusion)
      {Fusion Layer \\ \textbf{Quadrant Assignment}\\
       (Honest, Deceptive, Silent Violator, Overcautious)};

% ── Arrows ────────────────────────────────────────────────────────────────────
\draw[flow] (websites)   -- (behavioral);
\draw[flow] (websites)   -- (semantic);
\draw[flow] (behavioral) -- (bdetails);
\draw[flow] (semantic)   -- (sdetails);
\draw[flow] (bdetails)   -- (fusion);
\draw[flow] (sdetails)   -- (fusion);
\end{tikzpicture}

\caption{Dual-audit architecture. Each domain feeds two streams: the
\emph{behavioural} stream quantifies cookie practices via a Privacy-Violation
Score (PVS), and the \emph{semantic} stream uses large language models to
derive a rubric-based PolicyScore. A fusion layer combines both signals to
place sites into one of four CCPA-compliance quadrants.}
\label{fig:dual-audit-architecture}
\end{figure}


==> figures/industry-boxplot-per-website-by-type-with-N.tex <==
\begin{figure}[!t]
    \centering
    \includegraphics[width=1\linewidth]{figures/new_figures/box_ccpa_default_by_type.pdf}
    \caption{Distribution of cookies types per website across various sectors. The results reveal that Targeting cookies are common in for-profit industries.}
    \label{fig:industry-boxplot}
\end{figure}



==> figures/new_figures/consent-flow-cookies.tex <==
\begin{figure}[!t]
  \centering
  \includegraphics[width=0.88\linewidth]{figures/new_figures/cdf_websites_per_site_allcookies.pdf}
  \caption{Distribution of per-website cookie counts across consent stages (Initial, Accept, Reject). Websites set more cookies when user consents, but the difference is small.}
  \label{fig:consent-flow-cookies}
\end{figure}




==> figures/privacy-configs.tex <==
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=0.92\linewidth]{figures/new_figures/boxplot_all_types_by_config_all5_clean.pdf}
%     \caption{Distribution of cookie type counts per website across privacy configurations. The DNT and uBlock configurations observe a noticeable reduction in Targeting and Performance cookies.}
%     \label{fig:privacy-configs}
% \end{figure}



\begin{figure}[!t]
    \centering
    \includegraphics[width=0.92\linewidth]{figures/new_figures/boxplot_all_types_with_gpc.pdf}
    \caption{Distribution of cookie type counts per website across privacy configurations. The GPC and uBlock configurations observe a noticeable reduction in Targeting and Performance cookies.}
    \label{fig:privacy-configs}
\end{figure}



==> figures/related-work-comparison.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.91\linewidth]{figures/new_figures/Flower_Categories_v1-10.pdf}
    \caption{\name in the context of related research: Prior CCPA research has centered on dark patterns and compliance checks, whereas \name examines the less-studied domains of privacy policies and cookie-based tracking.}
    \label{fig:related-work-comparison}
\end{figure}



==> tables/cookie-classification.tex <==
\begin{table*}[tbp!]
    \centering
    \caption{Summary of Cookie Classification Outcomes}
    \label{tab:cookie-classification-summary}
    \begin{tabular}{|l|r|l|r|}
        \hline
        \textbf{Source Breakdown} & \textbf{Percent} & \textbf{Purpose Breakdown} & \textbf{Percent} \\
        \hline
        Combined Lookup Database & 66\% & Targeting & 37\% \\
        Manual Annotation / Uncategorized & 34\% & Performance & 32\% \\
        & & Functional & 22\% \\
        & & Strictly Necessary & 9\% \\
        \hline
    \end{tabular}
\end{table*}

==> tables/cookie-median-subjectivity.tex <==
% % --- Local helpers for Δ cells (do NOT modify your policy macros) ---
% % Map signed Δ in [-100,100] to the same red→green palette your policy table uses.


% \begin{table*}[!t]
% \centering
% \caption{Median cookie counts and relative change (\%$\Delta$) from the Default configuration across browsing modes, split by CCPA subjectivity.}

% \label{tab:cookie_median_subjectivity_gradient}
% \footnotesize
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lcccccccc}
% \toprule
% \textbf{Cookie Type} & \textbf{Configuration} & \textbf{Overall Median} & \textbf{\%$\Delta$ vs Default} & \textbf{Subjected Median} & \textbf{\%$\Delta$ Subj. vs Default} & \textbf{Non-Subj. Median} & \textbf{\%$\Delta$ Non-Subj. vs Default} \\
% \midrule
% \textbf{Targeting} & Default & 6 & \deltapolicyzero & 6 & \deltapolicyzero & 6 & \deltapolicyzero \\
%  & Do Not Track      & 6 & \deltapolicyzero   & 6 & \deltapolicyzero   & 5 & \deltapolicycell{-16.7} \\
%  & Block 3rd-Party   & 6 & \deltapolicyzero   & 6 & \deltapolicyzero   & 6 & \deltapolicyzero \\
%  & Allow 3rd-Party   & 6 & \deltapolicyzero   & 6 & \deltapolicyzero   & 6 & \deltapolicyzero \\
%  & uBlock            & 0 & \deltapolicycell{-100.0} & 0 & \deltapolicycell{-100.0} & 0 & \deltapolicycell{-100.0} \\
%  & GPC Enabled       & 3 & \deltapolicycell{-50.0}  & 2 & \deltapolicycell{-66.7}  & 3 & \deltapolicycell{-50.0} \\
% \midrule
% \textbf{Performance} & Default & 4 & \deltapolicyzero & 5 & \deltapolicyzero & 4 & \deltapolicyzero \\
%  & Do Not Track      & 4 & \deltapolicyzero   & 4 & \deltapolicycell{-20.0} & 4 & \deltapolicyzero \\
%  & Block 3rd-Party   & 4 & \deltapolicyzero   & 5 & \deltapolicyzero   & 4 & \deltapolicyzero \\
%  & Allow 3rd-Party   & 4 & \deltapolicyzero   & 4 & \deltapolicycell{-20.0} & 4 & \deltapolicyzero \\
%  & uBlock            & 0 & \deltapolicycell{-100.0} & 0 & \deltapolicycell{-100.0} & 0 & \deltapolicycell{-100.0} \\
%  & GPC Enabled       & 3 & \deltapolicycell{-25.0}  & 2 & \deltapolicycell{-60.0}  & 3 & \deltapolicycell{-25.0} \\
% \midrule
% \textbf{Functional} & Default & 2 & \deltapolicyzero & 3 & \deltapolicyzero & 2 & \deltapolicyzero \\
%  & Do Not Track      & 2 & \deltapolicyzero   & 2 & \deltapolicycell{-33.3} & 2 & \deltapolicyzero \\
%  & Block 3rd-Party   & 2 & \deltapolicyzero   & 2 & \deltapolicycell{-33.3} & 2 & \deltapolicyzero \\
%  & Allow 3rd-Party   & 3 & \deltapolicycell{50.0}   & 3 & \deltapolicyzero   & 2 & \deltapolicyzero \\
%  & uBlock            & 1 & \deltapolicycell{-50.0}  & 1 & \deltapolicycell{-66.7}  & 1 & \deltapolicycell{-50.0} \\
%  & GPC Enabled       & 2 & \deltapolicyzero   & 2 & \deltapolicycell{-33.3} & 2 & \deltapolicyzero \\
% \midrule
% \textbf{Strictly Necessary} & Default & 1 & \deltapolicyzero & 2 & \deltapolicyzero & 1 & \deltapolicyzero \\
%  & Do Not Track      & 1 & \deltapolicyzero   & 2 & \deltapolicyzero   & 1 & \deltapolicyzero \\
%  & Block 3rd-Party   & 1 & \deltapolicyzero   & 2 & \deltapolicyzero   & 1 & \deltapolicyzero \\
%  & Allow 3rd-Party   & 1 & \deltapolicyzero   & 2 & \deltapolicyzero   & 1 & \deltapolicyzero \\
%  & uBlock            & 1 & \deltapolicyzero   & 1 & \deltapolicycell{-50.0} & 0 & \deltapolicycell{-100.0} \\
%  & GPC Enabled       & 1 & \deltapolicyzero   & 1 & \deltapolicycell{-50.0} & 1 & \deltapolicyzero \\
% \midrule
% \textbf{Unknown} & Default & 6 & \deltapolicyzero & 7 & \deltapolicyzero & 5 & \deltapolicyzero \\
%  & Do Not Track      & 6 & \deltapolicyzero   & 6 & \deltapolicycell{-14.3} & 5 & \deltapolicyzero \\
%  & Block 3rd-Party   & 6 & \deltapolicyzero   & 7 & \deltapolicyzero   & 5 & \deltapolicyzero \\
%  & Allow 3rd-Party   & 6 & \deltapolicyzero   & 7 & \deltapolicyzero   & 5 & \deltapolicyzero \\
%  & uBlock            & 3 & \deltapolicycell{-50.0}  & 3 & \deltapolicycell{-57.1}  & 1 & \deltapolicycell{-80.0} \\
%  & GPC Enabled       & 4 & \deltapolicycell{-33.3}  & 4 & \deltapolicycell{-42.9}  & 3 & \deltapolicycell{-40.0} \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}

% \begin{table*}[!t]
% \centering
% \caption{Median cookie counts and relative change (\%$\Delta$) from the Default configuration across browsing modes, split by CCPA subjectivity.}
% \label{tab:cookie_median_subjectivity_gradient}
% \footnotesize
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lcccccccc}
% \toprule
% \textbf{Cookie Type} & \textbf{Configuration} & \textbf{Overall Median} & \textbf{\%$\Delta$ vs Default} & \textbf{Subjected Median} & \textbf{\%$\Delta$ Subj. vs Default} & \textbf{Non-Subj. Median} & \textbf{\%$\Delta$ Non-Subj. vs Default} \\
% \midrule
% \textbf{Targeting} & Default & 6 & \deltapolicyzero & 7 & \deltapolicyzero & 5 & \deltapolicyzero \\
%  & Do Not Track & 1 & \deltapolicycell{-83.3} & 1 & \deltapolicycell{-85.7} & 1 & \deltapolicycell{-80.0} \\
%  & Block 3rd-Party & 1 & \deltapolicycell{-83.3} & 1 & \deltapolicycell{-85.7} & 1 & \deltapolicycell{-80.0} \\
%  & uBlock & 1 & \deltapolicycell{-83.3} & 1 & \deltapolicycell{-85.7} & 1 & \deltapolicycell{-80.0} \\
%  & GPC Enabled & 2 & \deltapolicycell{-66.7} & 2 & \deltapolicycell{-71.4} & 0 & \deltapolicycell{-100.0} \\
% \midrule
% \textbf{Performance} & Default & 3 & \deltapolicyzero & 3 & \deltapolicyzero & 3 & \deltapolicyzero \\
%  & Do Not Track & 1 & \deltapolicycell{-66.7} & 1 & \deltapolicycell{-66.7} & 1 & \deltapolicycell{-66.7} \\
%  & Block 3rd-Party & 1 & \deltapolicycell{-66.7} & 1 & \deltapolicycell{-66.7} & 1 & \deltapolicycell{-66.7} \\
%  & uBlock & 0 & \deltapolicycell{-100.0} & 0 & \deltapolicycell{-100.0} & 0 & \deltapolicycell{-100.0} \\
%  & GPC Enabled & 1 & \deltapolicycell{-66.7} & 1 & \deltapolicycell{-66.7} & 0 & \deltapolicycell{-100.0} \\
% \midrule
% \textbf{Functional} & Default & 2 & \deltapolicyzero & 2 & \deltapolicyzero & 2 & \deltapolicyzero \\
%  & Do Not Track & 1 & \deltapolicycell{-50.0} & 1 & \deltapolicycell{-50.0} & 1 & \deltapolicycell{-50.0} \\
%  & Block 3rd-Party & 1 & \deltapolicycell{-50.0} & 1 & \deltapolicycell{-50.0} & 1 & \deltapolicycell{-50.0} \\
%  & uBlock & 1 & \deltapolicycell{-50.0} & 1 & \deltapolicycell{-50.0} & 1 & \deltapolicycell{-50.0} \\
%  & GPC Enabled & 1 & \deltapolicycell{-50.0} & 1 & \deltapolicycell{-50.0} & 1 & \deltapolicycell{-50.0} \\
% \midrule
% \textbf{Necessary} & Default & 2 & \deltapolicyzero & 2 & \deltapolicyzero & 2 & \deltapolicyzero \\
%  & Do Not Track & 1 & \deltapolicycell{-50.0} & 1 & \deltapolicycell{-50.0} & 1 & \deltapolicycell{-50.0} \\
%  & Block 3rd-Party & 1 & \deltapolicycell{-50.0} & 1 & \deltapolicycell{-50.0} & 1 & \deltapolicycell{-50.0} \\
%  & uBlock & 1 & \deltapolicycell{-50.0} & 1 & \deltapolicycell{-50.0} & 1 & \deltapolicycell{-50.0} \\
%  & GPC Enabled & 0 & \deltapolicycell{-100.0} & 0 & \deltapolicycell{-100.0} & 0 & \deltapolicycell{-100.0} \\
% \midrule
% \textbf{Unknown} & Default & 4 & \deltapolicyzero & 5 & \deltapolicyzero & 3 & \deltapolicyzero \\
%  & Do Not Track & 1 & \deltapolicycell{-75.0} & 1 & \deltapolicycell{-80.0} & 1 & \deltapolicycell{-66.7} \\
%  & Block 3rd-Party & 1 & \deltapolicycell{-75.0} & 1 & \deltapolicycell{-80.0} & 1 & \deltapolicycell{-66.7} \\
%  & uBlock & 1 & \deltapolicycell{-75.0} & 1 & \deltapolicycell{-80.0} & 0 & \deltapolicycell{-100.0} \\
%  & GPC Enabled & 1 & \deltapolicycell{-75.0} & 1 & \deltapolicycell{-80.0} & 1 & \deltapolicycell{-66.7} \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}


% \begin{table*}[!t]
% \centering
% \caption{Median cookie counts and relative change (\%$\Delta$) from the Default configuration across browsing modes, split by CCPA subjectivity.}
% \label{tab:cookie_median_subjectivity_gradient}
% \footnotesize
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lcccccccc}
% \toprule
% \textbf{Cookie Type} & \textbf{Configuration} & \textbf{Overall Median} & \textbf{\%$\Delta$ vs Default} & \textbf{Subjected Median} & \textbf{\%$\Delta$ Subj. vs Default} & \textbf{Non-Subj. Median} & \textbf{\%$\Delta$ Non-Subj. vs Default} \\
% \midrule
% \textbf{Targeting} & Default & 7 & \deltapolicyzero & 7 & \deltapolicyzero & 7 & \deltapolicyzero \\
%  & Do Not Track & 6 & \deltapolicycell{-14.3} & 6 & \deltapolicycell{-14.3} & 6 & \deltapolicycell{-14.3} \\
%  & Block 3rd-Party & 7 & \deltapolicycell{0.0} & 7 & \deltapolicycell{0.0} & 7 & \deltapolicycell{0.0} \\
%  & uBlock & 2 & \deltapolicycell{-71.4} & 2 & \deltapolicycell{-71.4} & 2 & \deltapolicycell{-71.4} \\
%  & GPC Enabled & 5 & \deltapolicycell{-28.6} & 5 & \deltapolicycell{-28.6} & 5 & \deltapolicycell{-28.6} \\
% \midrule
% \textbf{Performance} & Default & 4 & \deltapolicyzero & 5 & \deltapolicyzero & 4 & \deltapolicyzero \\
%  & Do Not Track & 4 & \deltapolicycell{0.0} & 4 & \deltapolicycell{-20.0} & 4 & \deltapolicycell{0.0} \\
%  & Block 3rd-Party & 5 & \deltapolicycell{25.0} & 5 & \deltapolicycell{0.0} & 4 & \deltapolicycell{0.0} \\
%  & uBlock & 2 & \deltapolicycell{-50.0} & 2 & \deltapolicycell{-60.0} & 2 & \deltapolicycell{-50.0} \\
%  & GPC Enabled & 4 & \deltapolicycell{0.0} & 4 & \deltapolicycell{-20.0} & 4 & \deltapolicycell{0.0} \\
% \midrule
% \textbf{Functional} & Default & 2 & \deltapolicyzero & 3 & \deltapolicyzero & 2 & \deltapolicyzero \\
%  & Do Not Track & 2 & \deltapolicycell{0.0} & 2 & \deltapolicycell{-33.3} & 2 & \deltapolicycell{0.0} \\
%  & Block 3rd-Party & 2 & \deltapolicycell{0.0} & 3 & \deltapolicycell{0.0} & 2 & \deltapolicycell{0.0} \\
%  & uBlock & 2 & \deltapolicycell{0.0} & 2 & \deltapolicycell{-33.3} & 1 & \deltapolicycell{-50.0} \\
%  & GPC Enabled & 2 & \deltapolicycell{0.0} & 2 & \deltapolicycell{-33.3} & 2 & \deltapolicycell{0.0} \\
% \midrule
% \textbf{Necessary} & Default & 2 & \deltapolicyzero & 2 & \deltapolicyzero & 1 & \deltapolicyzero \\
%  & Do Not Track & 2 & \deltapolicycell{0.0} & 2 & \deltapolicycell{0.0} & 1 & \deltapolicycell{0.0} \\
%  & Block 3rd-Party & 2 & \deltapolicycell{0.0} & 2 & \deltapolicycell{0.0} & 1 & \deltapolicycell{0.0} \\
%  & uBlock & 1 & \deltapolicycell{-50.0} & 1 & \deltapolicycell{-50.0} & 1 & \deltapolicycell{0.0} \\
%  & GPC Enabled & 2 & \deltapolicycell{0.0} & 2 & \deltapolicycell{0.0} & 1 & \deltapolicycell{0.0} \\
% \midrule
% \textbf{Unknown} & Default & 3 & \deltapolicyzero & 3 & \deltapolicyzero & 2 & \deltapolicyzero \\
%  & Do Not Track & 3 & \deltapolicycell{0.0} & 3 & \deltapolicycell{0.0} & 2 & \deltapolicycell{0.0} \\
%  & Block 3rd-Party & 3 & \deltapolicycell{0.0} & 3 & \deltapolicycell{0.0} & 2 & \deltapolicycell{0.0} \\
%  & uBlock & 3 & \deltapolicycell{0.0} & 3 & \deltapolicycell{0.0} & 2 & \deltapolicycell{0.0} \\
%  & GPC Enabled & 2 & \deltapolicycell{-33.3} & 3 & \deltapolicycell{0.0} & 2 & \deltapolicycell{0.0} \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}



% \begin{table*}[!t]
% \centering
% \caption{Median cookie counts and relative change (\%$\Delta$) from the Default configuration across browsing modes, split by CCPA subjectivity.}
% \label{tab:cookie_median_subjectivity_gradient}
% \footnotesize
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lcccccccc}
% \toprule
% \textbf{Cookie Type} & \textbf{Configuration} & \textbf{Overall Median} & \textbf{\%$\Delta$ vs Default} & \textbf{Subjected Median} & \textbf{\%$\Delta$ Subj. vs Default} & \textbf{Non-Subj. Median} & \textbf{\%$\Delta$ Non-Subj. vs Default} \\
% \midrule
% \textbf{Targeting} & Default & 7 & \deltapolicyzero & 7 & \deltapolicyzero & 7 & \deltapolicyzero \\
%  & Do Not Track & 6 & \deltapolicycell{-6.6} & 6 & \deltapolicycell{-7.7} & 6 & \deltapolicycell{-5.1} \\
%  & Block 3rd-Party & 7 & \deltapolicycell{0.3} & 7 & \deltapolicycell{-0.2} & 7 & \deltapolicycell{0.9} \\
%  & uBlock & 2 & \deltapolicycell{-81.1} & 2 & \deltapolicycell{-77.2} & 2 & \deltapolicycell{-86.7} \\
%  & GPC Enabled & 5 & \deltapolicycell{-32.1} & 5 & \deltapolicycell{-37.2} & 5 & \deltapolicycell{-24.9} \\
% \midrule
% \textbf{Performance} & Default & 4 & \deltapolicyzero & 5 & \deltapolicyzero & 4 & \deltapolicyzero \\
%  & Do Not Track & 4 & \deltapolicycell{-7.3} & 4 & \deltapolicycell{-8.9} & 4 & \deltapolicycell{-5.4} \\
%  & Block 3rd-Party & 5 & \deltapolicycell{-0.8} & 5 & \deltapolicycell{-1.1} & 4 & \deltapolicycell{-0.4} \\
%  & uBlock & 2 & \deltapolicycell{-81.2} & 2 & \deltapolicycell{-76.1} & 2 & \deltapolicycell{-87.3} \\
%  & GPC Enabled & 4 & \deltapolicycell{-29.2} & 4 & \deltapolicycell{-35.4} & 4 & \deltapolicycell{-21.9} \\
% \midrule
% \textbf{Functional} & Default & 2 & \deltapolicyzero & 3 & \deltapolicyzero & 2 & \deltapolicyzero \\
%  & Do Not Track & 2 & \deltapolicycell{-6.6} & 2 & \deltapolicycell{-6.4} & 2 & \deltapolicycell{-6.9} \\
%  & Block 3rd-Party & 2 & \deltapolicycell{-0.9} & 3 & \deltapolicycell{-1.0} & 2 & \deltapolicycell{-0.8} \\
%  & uBlock & 2 & \deltapolicycell{-47.9} & 2 & \deltapolicycell{-42.9} & 1 & \deltapolicycell{-55.6} \\
%  & GPC Enabled & 2 & \deltapolicycell{-23.6} & 2 & \deltapolicycell{-27.8} & 2 & \deltapolicycell{-16.8} \\
% \midrule
% \textbf{Necessary} & Default & 2 & \deltapolicyzero & 2 & \deltapolicyzero & 1 & \deltapolicyzero \\
%  & Do Not Track & 2 & \deltapolicycell{-3.8} & 2 & \deltapolicycell{-3.9} & 1 & \deltapolicycell{-3.7} \\
%  & Block 3rd-Party & 2 & \deltapolicycell{-1.1} & 2 & \deltapolicycell{-1.4} & 1 & \deltapolicycell{-0.5} \\
%  & uBlock & 1 & \deltapolicycell{-46.6} & 1 & \deltapolicycell{-37.4} & 1 & \deltapolicycell{-61.3} \\
%  & GPC Enabled & 2 & \deltapolicycell{-10.2} & 2 & \deltapolicycell{-14.7} & 1 & \deltapolicycell{-3.0} \\
% \midrule
% \textbf{Unknown} & Default & 3 & \deltapolicyzero & 3 & \deltapolicyzero & 3 & \deltapolicyzero \\
%  & Do Not Track & 3 & \deltapolicycell{-38.1} & 3 & \deltapolicycell{-4.5} & 2 & \deltapolicycell{-66.1} \\
%  & Block 3rd-Party & 3 & \deltapolicycell{-36.2} & 3 & \deltapolicycell{-0.4} & 2 & \deltapolicycell{-65.8} \\
%  & uBlock & 3 & \deltapolicycell{-55.1} & 3 & \deltapolicycell{-25.8} & 2 & \deltapolicycell{-79.4} \\
%  & GPC Enabled & 2 & \deltapolicycell{-46.4} & 3 & \deltapolicycell{-17.0} & 2 & \deltapolicycell{-70.9} \\
% \bottomrule
% \end{tabular}
% }
% \end{table*}


 % \begin{table*}[!t]
 %  \centering
 %  \caption{Median cookie counts and relative change (\%$\Delta$) from the Default configuration across browsing modes, split by CCPA subjectivity.
 %  Delta calculated from total cookie count reductions.}
 %  \label{tab:cookie_median_subjectivity_gradient}
 %  \footnotesize
 %  \resizebox{\textwidth}{!}{
 %  \begin{tabular}{lcccccccc}
 %  \toprule
 %  \textbf{Cookie Type} & \textbf{Configuration} & \textbf{Overall Median} & \textbf{\%$\Delta$ vs Default} & \textbf{Subjected Median} &
 %  \textbf{\%$\Delta$ Subj. vs Default} & \textbf{Non-Subj. Median} & \textbf{\%$\Delta$ Non-Subj. vs Default} \\
 %  \midrule
 %  \textbf{Targeting} & Default & 2 & \deltapolicyzero & 2 & \deltapolicyzero & 1 & \deltapolicyzero \\
 %   & Do Not Track & 1 & \deltapolicycell{-8.0} & 1 & \deltapolicycell{-8.7} & 1 & \deltapolicycell{-7.0} \\
 %   & Block 3rd-Party & 2 & \deltapolicycell{-1.3} & 2 & \deltapolicycell{-1.2} & 1 & \deltapolicycell{-1.4} \\
 %   & uBlock & 0 & \deltapolicycell{-81.3} & 0 & \deltapolicycell{-77.3} & 0 & \deltapolicycell{-86.8} \\
 %   & GPC Enabled & 1 & \deltapolicycell{-34.2} & 0 & \deltapolicycell{-39.3} & 1 & \deltapolicycell{-27.0} \\
 %  \midrule
 %  \textbf{Performance} & Default & 2 & \deltapolicyzero & 2 & \deltapolicyzero & 3 & \deltapolicyzero \\
 %   & Do Not Track & 2 & \deltapolicycell{-7.9} & 2 & \deltapolicycell{-9.3} & 2 & \deltapolicycell{-6.3} \\
 %   & Block 3rd-Party & 2 & \deltapolicycell{-1.5} & 2 & \deltapolicycell{-1.4} & 3 & \deltapolicycell{-1.7} \\
 %   & uBlock & 0 & \deltapolicycell{-81.4} & 0 & \deltapolicycell{-76.4} & 0 & \deltapolicycell{-87.3} \\
 %   & GPC Enabled & 2 & \deltapolicycell{-30.0} & 1 & \deltapolicycell{-36.1} & 2 & \deltapolicycell{-22.9} \\
 %  \midrule
 %  \textbf{Functional} & Default & 1 & \deltapolicyzero & 2 & \deltapolicyzero & 1 & \deltapolicyzero \\
 %   & Do Not Track & 1 & \deltapolicycell{-6.8} & 1 & \deltapolicycell{-6.7} & 1 & \deltapolicycell{-6.9} \\
 %   & Block 3rd-Party & 1 & \deltapolicycell{-1.2} & 2 & \deltapolicycell{-1.4} & 1 & \deltapolicycell{-1.0} \\
 %   & uBlock & 0 & \deltapolicycell{-48.0} & 1 & \deltapolicycell{-43.2} & 0 & \deltapolicycell{-55.6} \\
 %   & GPC Enabled & 1 & \deltapolicycell{-24.0} & 1 & \deltapolicycell{-28.1} & 1 & \deltapolicycell{-17.6} \\
 %  \midrule
 %  \textbf{Necessary} & Default & 1 & \deltapolicyzero & 1 & \deltapolicyzero & 0 & \deltapolicyzero \\
 %   & Do Not Track & 0 & \deltapolicycell{-3.9} & 1 & \deltapolicycell{-3.6} & 0 & \deltapolicycell{-4.4} \\
 %   & Block 3rd-Party & 1 & \deltapolicycell{-1.2} & 1 & \deltapolicycell{-1.2} & 0 & \deltapolicycell{-1.2} \\
 %   & uBlock & 0 & \deltapolicycell{-47.1} & 0 & \deltapolicycell{-38.0} & 0 & \deltapolicycell{-61.4} \\
 %   & GPC Enabled & 0 & \deltapolicycell{-11.6} & 0 & \deltapolicycell{-16.2} & 0 & \deltapolicycell{-4.4} \\
 %  \midrule
 %  \textbf{Unknown} & Default & 1 & \deltapolicyzero & 1 & \deltapolicyzero & 0 & \deltapolicyzero \\
 %   & Do Not Track & 1 & \deltapolicycell{-4.4} & 1 & \deltapolicycell{-5.0} & 0 & \deltapolicycell{-3.1} \\
 %   & Block 3rd-Party & 1 & \deltapolicycell{-1.4} & 1 & \deltapolicycell{-1.6} & 0 & \deltapolicycell{-1.1} \\
 %   & uBlock & 0 & \deltapolicycell{-30.6} & 1 & \deltapolicycell{-26.5} & 0 & \deltapolicycell{-40.3} \\
 %   & GPC Enabled & 0 & \deltapolicycell{-18.0} & 1 & \deltapolicycell{-18.5} & 0 & \deltapolicycell{-16.7} \\
 %  \bottomrule
 %  \end{tabular}
 %  }
 %  \end{table*}

  %  \begin{table*}[!t]
  % \centering
  % \caption{Median cookie counts and relative change (\%$\Delta$) from the Default configuration across browsing modes, split by CCPA subjectivity.
  % Medians calculated only for websites serving each cookie type. Delta calculated from total cookie count reductions.}
  % \label{tab:cookie_median_subjectivity_gradient}
  % \footnotesize
  % \resizebox{\textwidth}{!}{
  % \begin{tabular}{lcccccccc}
  % \toprule
  % \textbf{Cookie Type} & \textbf{Configuration} & \textbf{Overall Median} & \textbf{\%$\Delta$ vs Default} & \textbf{Subjected Median} &
  % \textbf{\%$\Delta$ Subj. vs Default} & \textbf{Non-Subj. Median} & \textbf{\%$\Delta$ Non-Subj. vs Default} \\
  % \midrule
  % \textbf{Targeting} & Default & 7 & \deltapolicyzero & 7 & \deltapolicyzero & 7 & \deltapolicyzero \\
  %  & Do Not Track & 6 & \deltapolicycell{-8.0} & 6 & \deltapolicycell{-8.7} & 6 & \deltapolicycell{-7.0} \\
  %  & Block 3rd-Party & 7 & \deltapolicycell{-1.3} & 7 & \deltapolicycell{-1.2} & 6 & \deltapolicycell{-1.4} \\
  %  & uBlock & 1 & \deltapolicycell{-81.3} & 1 & \deltapolicycell{-77.3} & 0 & \deltapolicycell{-86.8} \\
  %  & GPC Enabled & 4 & \deltapolicycell{-34.2} & 4 & \deltapolicycell{-39.3} & 5 & \deltapolicycell{-27.0} \\
  % \midrule
  % \textbf{Performance} & Default & 4 & \deltapolicyzero & 5 & \deltapolicyzero & 4 & \deltapolicyzero \\
  %  & Do Not Track & 4 & \deltapolicycell{-7.9} & 4 & \deltapolicycell{-9.3} & 4 & \deltapolicycell{-6.3} \\
  %  & Block 3rd-Party & 4 & \deltapolicycell{-1.5} & 5 & \deltapolicycell{-1.4} & 4 & \deltapolicycell{-1.7} \\
  %  & uBlock & 0 & \deltapolicycell{-81.4} & 1 & \deltapolicycell{-76.4} & 0 & \deltapolicycell{-87.3} \\
  %  & GPC Enabled & 3 & \deltapolicycell{-30.0} & 3 & \deltapolicycell{-36.1} & 4 & \deltapolicycell{-22.9} \\
  % \midrule
  % \textbf{Functional} & Default & 2 & \deltapolicyzero & 3 & \deltapolicyzero & 2 & \deltapolicyzero \\
  %  & Do Not Track & 2 & \deltapolicycell{-6.8} & 2 & \deltapolicycell{-6.7} & 2 & \deltapolicycell{-6.9} \\
  %  & Block 3rd-Party & 2 & \deltapolicycell{-1.2} & 3 & \deltapolicycell{-1.4} & 2 & \deltapolicycell{-1.0} \\
  %  & uBlock & 1 & \deltapolicycell{-48.0} & 1 & \deltapolicycell{-43.2} & 1 & \deltapolicycell{-55.6} \\
  %  & GPC Enabled & 2 & \deltapolicycell{-24.0} & 2 & \deltapolicycell{-28.1} & 2 & \deltapolicycell{-17.6} \\
  % \midrule
  % \textbf{Necessary} & Default & 2 & \deltapolicyzero & 2 & \deltapolicyzero & 1 & \deltapolicyzero \\
  %  & Do Not Track & 1 & \deltapolicycell{-3.9} & 2 & \deltapolicycell{-3.6} & 1 & \deltapolicycell{-4.4} \\
  %  & Block 3rd-Party & 2 & \deltapolicycell{-1.2} & 2 & \deltapolicycell{-1.2} & 1 & \deltapolicycell{-1.2} \\
  %  & uBlock & 1 & \deltapolicycell{-47.1} & 1 & \deltapolicycell{-38.0} & 1 & \deltapolicycell{-61.4} \\
  %  & GPC Enabled & 1 & \deltapolicycell{-11.6} & 1 & \deltapolicycell{-16.2} & 1 & \deltapolicycell{-4.4} \\
  % \midrule
  % \textbf{Unknown} & Default & 3 & \deltapolicyzero & 3 & \deltapolicyzero & 2 & \deltapolicyzero \\
  %  & Do Not Track & 3 & \deltapolicycell{-4.4} & 3 & \deltapolicycell{-5.0} & 2 & \deltapolicycell{-3.1} \\
  %  & Block 3rd-Party & 3 & \deltapolicycell{-1.4} & 3 & \deltapolicycell{-1.6} & 2 & \deltapolicycell{-1.1} \\
  %  & uBlock & 2 & \deltapolicycell{-30.6} & 3 & \deltapolicycell{-26.5} & 1 & \deltapolicycell{-40.3} \\
  %  & GPC Enabled & 2 & \deltapolicycell{-18.0} & 3 & \deltapolicycell{-18.5} & 2 & \deltapolicycell{-16.7} \\
  % \bottomrule
  % \end{tabular}
  % }
  % \end{table*}

%   \begin{table*}[!t]
%   \centering
%   \caption{Median cookie counts and relative change (\%$\Delta$) from the Default configuration across browsing modes, split by CCPA subjectivity.
%   Medians calculated only for websites serving each cookie type. Delta calculated from total cookie count reductions.}
%   \label{tab:cookie_median_subjectivity_gradient}
%   \footnotesize
%   \resizebox{\textwidth}{!}{
%   \begin{tabular}{lcccccccc}
%   \toprule
%   \textbf{Cookie Type} & \textbf{Configuration} & \textbf{Overall Median} & \textbf{\%$\Delta$ vs Default} & \textbf{Subjected Median} &
%   \textbf{\%$\Delta$ Subj. vs Default} & \textbf{Non-Subj. Median} & \textbf{\%$\Delta$ Non-Subj. vs Default} \\
%   \midrule
%   \textbf{Targeting} & Default & 7 & \deltapolicyzero & 7 & \deltapolicyzero & 7 & \deltapolicyzero \\
%    & Do Not Track & 6 & \deltapolicycell{-8.0} & 6 & \deltapolicycell{-8.7} & 6 & \deltapolicycell{-7.0} \\
%    & Block 3rd-Party & 7 & \deltapolicycell{-1.3} & 7 & \deltapolicycell{-1.2} & 7 & \deltapolicycell{-1.4} \\
%    & uBlock & 2 & \deltapolicycell{-81.3} & 2 & \deltapolicycell{-77.3} & 2 & \deltapolicycell{-86.8} \\
%    & GPC Enabled & 5 & \deltapolicycell{-34.2} & 5 & \deltapolicycell{-39.3} & 5 & \deltapolicycell{-27.0} \\
%   \midrule
%   \textbf{Performance} & Default & 4 & \deltapolicyzero & 5 & \deltapolicyzero & 4 & \deltapolicyzero \\
%    & Do Not Track & 4 & \deltapolicycell{-7.9} & 4 & \deltapolicycell{-9.3} & 4 & \deltapolicycell{-6.3} \\
%    & Block 3rd-Party & 5 & \deltapolicycell{-1.5} & 5 & \deltapolicycell{-1.4} & 4 & \deltapolicycell{-1.7} \\
%    & uBlock & 2 & \deltapolicycell{-81.4} & 2 & \deltapolicycell{-76.4} & 2 & \deltapolicycell{-87.3} \\
%    & GPC Enabled & 4 & \deltapolicycell{-30.0} & 4 & \deltapolicycell{-36.1} & 4 & \deltapolicycell{-22.9} \\
%   \midrule
%   \textbf{Functional} & Default & 2 & \deltapolicyzero & 3 & \deltapolicyzero & 2 & \deltapolicyzero \\
%    & Do Not Track & 2 & \deltapolicycell{-6.8} & 2 & \deltapolicycell{-6.7} & 2 & \deltapolicycell{-6.9} \\
%    & Block 3rd-Party & 2 & \deltapolicycell{-1.2} & 3 & \deltapolicycell{-1.4} & 2 & \deltapolicycell{-1.0} \\
%    & uBlock & 2 & \deltapolicycell{-48.0} & 2 & \deltapolicycell{-43.2} & 1 & \deltapolicycell{-55.6} \\
%    & GPC Enabled & 2 & \deltapolicycell{-24.0} & 2 & \deltapolicycell{-28.1} & 2 & \deltapolicycell{-17.6} \\
%   \midrule
%   \textbf{Necessary} & Default & 2 & \deltapolicyzero & 2 & \deltapolicyzero & 1 & \deltapolicyzero \\
%    & Do Not Track & 2 & \deltapolicycell{-3.9} & 2 & \deltapolicycell{-3.6} & 1 & \deltapolicycell{-4.4} \\
%    & Block 3rd-Party & 2 & \deltapolicycell{-1.2} & 2 & \deltapolicycell{-1.2} & 1 & \deltapolicycell{-1.2} \\
%    & uBlock & 1 & \deltapolicycell{-47.1} & 1 & \deltapolicycell{-38.0} & 1 & \deltapolicycell{-61.4} \\
%    & GPC Enabled & 2 & \deltapolicycell{-11.6} & 2 & \deltapolicycell{-16.2} & 1 & \deltapolicycell{-4.4} \\
%   \midrule
%   \textbf{Unknown} & Default & 3 & \deltapolicyzero & 4 & \deltapolicyzero & 3 & \deltapolicyzero \\
%    & Do Not Track & 3 & \deltapolicycell{-74.8} & 3 & \deltapolicycell{-57.8} & 2 & \deltapolicycell{-87.1} \\
%    & Block 3rd-Party & 3 & \deltapolicycell{-74.1} & 3 & \deltapolicycell{-56.3} & 2 & \deltapolicycell{-86.8} \\
%    & uBlock & 3 & \deltapolicycell{-81.7} & 3 & \deltapolicycell{-67.4} & 2 & \deltapolicycell{-92.1} \\
%    & GPC Enabled & 2 & \deltapolicycell{-78.4} & 3 & \deltapolicycell{-63.8} & 2 & \deltapolicycell{-88.9} \\
%   \bottomrule
%   \end{tabular}
%   }
% \end{table*}

\begin{table*}[!t]
  \centering
  \caption{Median cookie counts and relative change (\%$\Delta$) from the Default configuration across browsing modes, split by CCPA subjectivity.
  Medians calculated only for websites serving each cookie type. Delta calculated from total cookie count reductions.}
  \label{tab:cookie_median_subjectivity_gradient}
  \footnotesize
  \resizebox{\textwidth}{!}{
  \begin{tabular}{lcccccccc}
  \toprule
  \textbf{Cookie Type} & \textbf{Configuration} & \textbf{Overall Median} & \textbf{\%$\Delta$ vs Default} & \textbf{Subjected Median} &
  \textbf{\%$\Delta$ Subj. vs Default} & \textbf{Non-Subj. Median} & \textbf{\%$\Delta$ Non-Subj. vs Default} \\
  \midrule
  \textbf{Targeting} & Default & 7 & \deltapolicyzero & 7 & \deltapolicyzero & 7 & \deltapolicyzero \\
   & Do Not Track & 6 & \deltapolicycell{-38.1} & 6 & \deltapolicycell{-26.7} & 6 & \deltapolicycell{-49.0} \\
   & Block 3rd-Party & 7 & \deltapolicycell{-33.5} & 7 & \deltapolicycell{-20.7} & 7 & \deltapolicycell{-45.9} \\
   & uBlock & 2 & \deltapolicycell{-87.3} & 2 & \deltapolicycell{-81.7} & 2 & \deltapolicycell{-92.7} \\
   & GPC Enabled & 5 & \deltapolicycell{-55.7} & 5 & \deltapolicycell{-51.2} & 5 & \deltapolicycell{-60.0} \\
  \midrule
  \textbf{Performance} & Default & 4 & \deltapolicyzero & 5 & \deltapolicyzero & 4 & \deltapolicyzero \\
   & Do Not Track & 4 & \deltapolicycell{-12.1} & 4 & \deltapolicycell{-12.4} & 4 & \deltapolicycell{-11.7} \\
   & Block 3rd-Party & 5 & \deltapolicycell{-6.0} & 5 & \deltapolicycell{-4.8} & 4 & \deltapolicycell{-7.4} \\
   & uBlock & 2 & \deltapolicycell{-82.3} & 2 & \deltapolicycell{-77.3} & 2 & \deltapolicycell{-88.1} \\
   & GPC Enabled & 4 & \deltapolicycell{-33.3} & 4 & \deltapolicycell{-38.2} & 4 & \deltapolicycell{-27.6} \\
  \midrule
  \textbf{Functional} & Default & 2 & \deltapolicyzero & 2 & \deltapolicyzero & 2 & \deltapolicyzero \\
   & Do Not Track & 2 & \deltapolicycell{-11.0} & 2 & \deltapolicycell{-9.7} & 2 & \deltapolicycell{-13.1} \\
   & Block 3rd-Party & 2 & \deltapolicycell{-5.7} & 3 & \deltapolicycell{-4.5} & 2 & \deltapolicycell{-7.6} \\
   & uBlock & 2 & \deltapolicycell{-50.4} & 2 & \deltapolicycell{-45.0} & 1 & \deltapolicycell{-58.5} \\
   & GPC Enabled & 2 & \deltapolicycell{-27.5} & 2 & \deltapolicycell{-30.4} & 2 & \deltapolicycell{-23.0} \\
  \midrule
  \textbf{Necessary} & Default & 2 & \deltapolicyzero & 2 & \deltapolicyzero & 2 & \deltapolicyzero \\
   & Do Not Track & 2 & \deltapolicycell{-19.4} & 2 & \deltapolicycell{-13.3} & 1 & \deltapolicycell{-27.5} \\
   & Block 3rd-Party & 2 & \deltapolicycell{-16.8} & 2 & \deltapolicycell{-10.7} & 1 & \deltapolicycell{-25.0} \\
   & uBlock & 1 & \deltapolicycell{-53.6} & 1 & \deltapolicycell{-42.8} & 1 & \deltapolicycell{-68.2} \\
   & GPC Enabled & 2 & \deltapolicycell{-26.0} & 2 & \deltapolicycell{-24.4} & 1 & \deltapolicycell{-28.1} \\
  \midrule
  \textbf{Unknown} & Default & 3 & \deltapolicyzero & 3 & \deltapolicyzero & 2 & \deltapolicyzero \\
   & Do Not Track & 3 & \deltapolicycell{-65.9} & 3 & \deltapolicycell{-47.3} & 2 & \deltapolicycell{-81.7} \\
   & Block 3rd-Party & 3 & \deltapolicycell{-64.9} & 3 & \deltapolicycell{-45.5} & 2 & \deltapolicycell{-81.4} \\
   & uBlock & 2 & \deltapolicycell{-75.0} & 3 & \deltapolicycell{-58.9} & 2 & \deltapolicycell{-88.8} \\
   & GPC Enabled & 2 & \deltapolicycell{-70.8} & 3 & \deltapolicycell{-54.9} & 2 & \deltapolicycell{-84.3} \\
  \bottomrule
  \end{tabular}
  }
\end{table*}

==> tables/privacy-configs.tex <==

\begin{table}[!t]
\centering
\scriptsize
\caption{\textbf{\name's Browser Privacy Configurations.}}
\label{tab:privacy-configs}
\begin{tabular}{l l}
\toprule
\textbf{Configuration} & \textbf{Mechanism} \\
\midrule
Default Chrome
    & Baseline browser with default settings \\
\cellcolor{gray!20}Block 3rd-Party Cookies
    & \cellcolor{gray!20}Browser blocks cross-site cookies \\
Do Not Track (DNT)
    & Sends DNT header signal \\
\cellcolor{gray!20}Global Privacy Control (GPC)
    & \cellcolor{gray!20}Sends Sec-GPC: 1 header and JS signal \\
uBlock Origin
    & Blocks known trackers and ads~\cite{easylist} \\
\cellcolor{gray!20}Consent-O-Matic
    & \cellcolor{gray!20}Automates consent banner interaction \\
\bottomrule
\end{tabular}
\end{table}

